Red Teaming Visual Language Models

VLMs (Vision-Language Models) extend the capabilities of LLMs (Large Language Models) to accept multimodal inputs. Since it has been verified that LLMs can be induced to generate harmful or inaccurate content through specific test cases (termed as Red Teaming), how VLMs perform in similar scenarios, especially with their combination of textual and visual inputs, remains a question. To explore this problem, we present a novel red teaming dataset RTVLM, which encompasses 10 subtasks (e.g., image misleading, multi-modal jail-breaking, face fairness, etc) under 4 primary aspects (faithfulness, privacy, safety, fairness). Our RTVLM is the first red-teaming dataset to benchmark current VLMs in terms of these 4 different aspects. Detailed analysis shows that 10 prominent open-sourced VLMs struggle with the red teaming in different degrees and have up to 31% performance gap with GPT-4V. Additionally, we simply apply red teaming alignment to LLaVA-v1.5 with Supervised Fine-tuning (SFT) using RTVLM, and this bolsters the models' performance with 10% in RTVLM test set, 13% in MM-Hal, and without noticeable decline in MM-Bench, overpassing other LLaVA-based models with regular alignment data. This reveals that current open-sourced VLMs still lack red teaming alignment. Our code and datasets will be open-source.

==> 05defense.tex <==
\section{Harm Reduce}
\subsection{Harm reduce methods}
% \paragraph{SFT Methods}
\begin{table}[!h]
\setlength{\tabcolsep}{3.8pt}
% \captionsetup{skip=4pt}
\centering
\small
\begin{tabular}{l|cccccccc}
% \toprule
% & \multicolumn{4}{c}{Misleading}& \multicolumn{1}{c}{Jailbreak}    & \multicolumn{1}{c}{Harmful Contents} \\
% \cmidrule(lr){2-5}
% \cmidrule(lr){6}
% \cmidrule(lr){7} \\
\toprule 
 & \textbf{MMBench} &\textbf{MMHAL} &\textbf{RTVLM}_{t}  \\
\midrule

LLaVA-RLHF  & 64.2   &2.09   & 7.82  \\
LLaVA-SFT   &  63.8      &2.16   & 8.17\\
LLaVA-v1.5    &64.3    &2.30  & 8.38 \\

\quad + RedTeaming &66.8  &2.55   &\textbf{8.54}\\
LLaVA-v1.5-SG  & \textbf{71.9}   &2.28   &8.37\\
\quad  + RedTeaming     & 71.2     &\textbf{2.59}  & 8.51\\
% & - & - & - & - & - & - & - & - & - & - \\

% & - & - & - & - & - & - & - & - & - & - \\
\bottomrule
\end{tabular}
\caption{MMbench, MMHallucination bench and RTVLM test set Results Table with 7B-size LLaVA series model. LLaVA-v1.5-SG stands for ShareGPT4V SFT version of LLaVA-v1.5.}
\label{table:my_label}
\end{table}
We sampled a portion of the \dataset data and related GPT4V generated data to use as RedTeaming SFT data, to test if it can reduce the model's harm and hallucinations, while also assessing if it impacts other aspects of the model's performance. We compared models in the LLaVA series, including LLaVA-RLHF, LLaVA-SFT, LLaVA-v1.5, and LLaVA-v1.5-ShareGPT4V. For the latter two, we used sampled \dataset data for SFT. Following the LoRA approach, we applied LoRA~\citep{hu2021lora} to the query value vectors in the attention mechanism for $3$ epochs and with a lower learning rate of 1$e$-5 and a warmup stage of $1000$ steps. 
All experiments are conducted with 1 single NVIDIA 80GB A100 GPUs. It took about 0.5 hours to complete the SFT pipeline.

% \paragraph{DPO methods}
% % add some preference data results
% add in the future version
\subsection{Harm reduce results}
As shown in Table 5, training LLaVA1.5 and LLaVA1.5-ShareGPT4V with sampled \dataset data results in a obvious improvement on MMhal-B and test set of \dataset, while performance on MMbench remains largely unchanged. This indicates that using RTVLM as SFT data can enhance the safety and robustness of the model without major changes in downstream task performance. Compared to using ShareGPT4V as SFT data, employing sampled \dataset data noticeably improves the model's performance on MMhal. Furthermore, utilizing both Sharegpt4v and \dataset data achieves better results in terms of both performance and safety.

% In contrast, the second table focuses on the general task performance of the models, comparing them with baseline models on standard tasks as represented by MMBench and MMHAL-B metrics. The results here are particularly noteworthy as they indicate that the improvements in handling red teaming scenarios do not come at the cost of general task performance. 
% % The LLaVA1.5-SFT and its fine-tuned variant maintain a competitive performance level in these general tasks, with scores comparable to, or slightly better than, the baseline LLaVA1.5-RLHF model. This finding is crucial as it underscores the balanced nature of our approach: enhancing the models' ability to counteract red teaming without compromising their effectiveness in routine tasks. This balance is critical for the practical deployment of MLMs, ensuring they remain versatile and reliable across a broad spectrum of applications.

